Sequence-to-Sequence Modeling for Action Identification at High Temporal Resolution

Automatic action identification from video and kinematic data is an important machine learning problem with applications ranging from robotics to smart health. Most existing works focus on identifying coarse actions such as running, climbing, or cutting a vegetable, which have relatively long durations. This is an important limitation for applications that require the identification of subtle motions at high temporal resolution. For example, in stroke recovery, quantifying rehabilitation dose requires differentiating motions with sub-second durations. Our goal is to bridge this gap. To this end, we introduce a large-scale, multimodal dataset, StrokeRehab, as a new action-recognition benchmark that includes subtle short-duration actions labeled at a high temporal resolution. These short-duration actions are called functional primitives, and consist of reaches, transports, repositions, stabilizations, and idles. The dataset consists of high-quality Inertial Measurement Unit sensors and video data of 41 stroke-impaired patients performing activities of daily living like feeding, brushing teeth, etc. We show that current state-of-the-art models based on segmentation produce noisy predictions when applied to these data, which often leads to overcounting of actions. To address this, we propose a novel approach for high-resolution action identification, inspired by speech-recognition techniques, which is based on a sequence-to-sequence model that directly predicts the sequence of actions. This approach outperforms current state-of-the-art methods on the StrokeRehab dataset, as well as on the standard benchmark datasets 50Salads, Breakfast, and Jigsaws.

==> old_files/old_results.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Performance metrics}
\label{sec:metrics}
\subsubsection{Edit score and action error rate}
Define the edit score.
Taking inspiration from automatic speech recognition literature, we use a modified version of Action Error Rate - action error rate to measure the performance of our models.

Since we are interested in the order prediction, we choose edit score and action error rate as our metric. Action error rate, similar to Action Error Rate, is typically used in speech recognition and unlike edit score, it penalizes the longer predictions of the model. The edit score on the other hand is lenient when the model over-predicts. In addition to edit score and action error rate, we also keep track of the counts of the action movements using TPR and FDR.

\subsubsection{True positive rate and False discovery rate}
We also evaluated the model performance using the true positive rate (TPR) and the false discovery rate (FDR). To compute these quantities we compared the estimated sequence to the ground truth actions to determine the number of actions that AERe correctly identified, incorrectly identified (e.g. the model estimates a transport, but the ground truth is a reach), missed (an action present in the ground truth is not present in the estimate), or spurious (an action present in the estimate is not present in the ground truth). The TPR is the ratio between the correctly-identified actions and the total ground-truth actions. The FDR is the ratio between the wrong predictions (incorrectly identified and spurious) and the total estimated actions.

\subsection{Experiment Setting}
% For the experiment of Seq2seq refinement on the ASRF prediction

To enable more stable training on the long input sequence, we divide a whole sequence to small windows with overlap during training. The seq2seq model is applied on top of each time window. During inference, each sequence is divided to time windows without overlap. We then concatenate the result for each time window and remove the duplicate. If the last time window in the the whole sequence is shorter than the required time window size, zero padding is applied to achieve the same length. 

The prediction of each step is conditioned on the previous actions for the seq2seq model. During the inference, we do not have the ground truth of the previous step and the prediction can suffer if the model was not trained to be resilient to the bad prediction. To ameliorate such effect, we follow the trick in~\cite{bengio2015scheduled} during training. Instead of always feeding the ground truth, we leave some probability to sample from the previous action distribution and take that as the input to the model. 


For Jigsaws, 50 salads and breakfast dataset, we follow the setting in ASRF. We use a separate small validation set divided from the training set of each fold, and test the performance on the val set of that fold. We select the model according to the best Action Error Rate (AER) on the validation set, then average the result of all the folds. 


For the stroke dataset, there is a common leave out test set for all the 4 folds.  For each fold, we select the model according to the best Action Error Rate (AER) on the validation set and test the performance on the leave out test set. We ensemble the prediction of the models trained on 4 folds on the common test set. For the action segmentation model prediction, we take the average of the probability of the 4 folds. For the seq2seq model, since the decoding on the next primitive depends on the prediction of the previous step. Therefore, the prediction at a specific time step for individual model is conditioned on the average predictions of the four models from the previous step. 







\subsection{Baseline Models}

ASRF model is currently the state-of-the-art model for action segmentation. Therefore, we take it as a strong baseline. Based on the MS-TCN backbone, it produces raw frame-wise predictions. Besides, it trained a boundary classification model to produce boundary information, which is then used to refine the raw frame-wise prediction. Additionally, we report a non-parametric way to conduct refinement of top of the raw frame-wise prediction by smoothing windows. 






% \subsection{Previous Sota models}
% \label{sec:sota_model}

% Boundary aware method?

\subsection{Result}
\label{sec:seq2seq_model}
% Seq2seq on video data

% a. Extract features using pretrained models (like on kinetic data)

% b. Extract features using models that predicts label for the center time step of the window (I3D and X3D)

% c. Prob. prediction of the video segmentation model in the seq2seq arch. 

% \begin{table}[]
% \centering
% % \resizebox{0.9\linewidth}{!}{
% \begin{tabular}{ c | c  | c| c| c}
% \toprule
%     & \multicolumn{1}{c}{Edit Score} & \multicolumn{1}{c}{Action Error Rate} &  \multicolumn{1}{c}{FDR} & \multicolumn{1}{c}{TPR}\\
    
% % \cmidrule{4-7}
% %\midrule
% \midrule[0.7pt]
% {Asrf (before refinement)}  & 61.6 & 0.48 &0.17&0.67  \\
% {Asrf (after refinement)} & {56.3} & 0.50&\textbf{0.11}&0.59 \\
% {Seq2seq (on Asrf prediction)} & \textbf{65.5}& \textbf{0.47}  & 0.23&\textbf{0.72}\\
% {Seq2seq (on raw video feature data)} & {63.4} &  {0.50} &0.24&0.71 \\
% \bottomrule
% \end{tabular}
% % }
%     \caption{Stroke video dataset}
%     \label{tab:my_label1}
% \end{table}

% \begin{table}[]
% \centering
% \resizebox{1\linewidth}{!}{
% \begin{tabular}{ c | c  | c| c| c}
% \toprule
%     & \multicolumn{1}{c}{Edit Score} & \multicolumn{1}{c}{Action Error Rate} &  \multicolumn{1}{c}{FDR} & \multicolumn{1}{c}{TPR}\\
    
% % \cmidrule{4-7}
% %\midrule
% \midrule[0.7pt]
% % {Asrf (before refinement)}  & 61.6 (60.0 - 63.0) & 0.400 (0.380, 0.419) &0.133 (0.121, 0.145) &0.630 (0.612, 0.652)  \\
% {Asrf (before refinement)}  & 62.2 (60.8 - 63.6) & 0.392 (0.371, 0.413) &0.148 (0.135, 0.161) &0.643 (0.622, 0.664)  \\
% % {Asrf (after refinement)} & {57.3 (55.8 - 58.9)} & 0.448 (0.429 - 0.467) & 0.113 (0.101 - 0.125) &0.567 (0.548 - 0.587) \\
% {Asrf (Boundary refinement)} & {58.7 (57.3 - 60.2)} & 0.436 (0.417 - 0.456) & 0.126 (0.113 - 0.139) &0.585 (0.566 - 0.605) \\
% {Asrf (Smoothing window refinement)}  & 62.2 (60.8 - 63.6) & 0.392 (0.371, 0.413) &0.148 (0.135, 0.161) &0.643 (0.622, 0.664)  \\
% {Seq2seq (on Asrf prediction ( best individual) )} & \textbf{66.9 (65.6 - 68.1)}& \textbf{0.333 (0.317 - 0.349)}  & 0.213 (0.203 - 0.223) &\textbf{0.736 (0.725 - 0.746)}\\
% {Seq2seq (on Asrf prediction ( average ensemble) )} & {64.2 (62.9 - 65.5)}& {0.353 (0.337 - 0.369)}  & 0.178 (0.168 - 0.188) &{0.680} (0.671 - 0.692)\\
% {Seq2seq (on Asrf prediction ( ensemble pred) )} & {67.6 (66.4 - 68.8)}& {0.322 (0.307 - 0.339)}  & 0.211 (0.200 - 0.221) &{0.743} (0.732 - 0.753)\\
% % {Seq2seq (on raw video feature data)} & {63.4} &  {0.50} &0.24&0.71 \\
% {Seq2seq (on raw video feature data)} best individual & {64.8 (63.6 - 66.0))} &  {0.348 (0.334 - 0.364) } &0.212 (0.202 - 0.223) &0.709 (0.698 - 0.720) \\
% {Seq2seq (on raw video feature data)} average ensemble & {61.8 (60.4 - 63.2))} &  {0.373 (0.357 - 0.390) } &0.175 (0.165 - 0.184) &0.655 (0.643 - 0.666) \\
% {Seq2seq (on raw video feature data)} ensemble pred & {66.6 (65.4 - 67.9))} &  {0.329 (0.312 - 0.345) } &0.216 (0.207 - 0.226) &0.734 (0.722 - 0.744) \\
% \bottomrule
% \end{tabular}
% }
%     \caption{Stroke video dataset: we select the model according to the best Action Error Rate on the validation set and test the performance on the leave out testset. }
%     \label{tab:my_label1}
% \end{table}


% \begin{table}[]
% \centering
% \resizebox{1\linewidth}{!}{
% \begin{tabular}{ c | c  | c| c| c}
% \toprule
%     & \multicolumn{1}{c}{Edit Score} & \multicolumn{1}{c}{Action Error Rate} &  \multicolumn{1}{c}{FDR} & \multicolumn{1}{c}{TPR}\\
    
% % \cmidrule{4-7}
% %\midrule
% \midrule[0.7pt]
% {Asrf (before refinement)}  & 62.2 (60.8 - 63.6) & 0.392 (0.371 - 0.413) &0.148 (0.135 - 0.161) &0.643 (0.622- 0.664)  \\
% {Asrf (Boundary refinement)} & {58.7 (57.3 - 60.2)} & 0.436 (0.417 - 0.456) & \textbf{0.126 (0.113 - 0.139)} &  0.585 (0.566 - 0.605) \\
% {Asrf (Smoothing window refinement)}  & 62.2 (60.8 - 63.6) & 0.392 (0.371, 0.413) & 0.148 (0.135 - 0.161) &0.643 (0.622, 0.664)  \\
% {Asrf (Seq2seq refinement) } & \textbf{{67.6 (66.4 - 68.8)}}& \textbf{{0.322 (0.307 - 0.339)}}  & 0.211 (0.200 - 0.221) &\textbf{{0.743} (0.732 - 0.753)}\\
% \midrule[0.7pt]

% {Seq2seq (on raw video feature data)} ensemble pred & {66.6 (65.4 - 67.9)} & {0.329 (0.312 - 0.345)} &0.216 (0.207 - 0.226) &0.734 (0.722 - 0.744) \\
% \bottomrule
% \end{tabular}
% }
%     \caption{Stroke video dataset: we select the model according to the best Action Error Rate (AER) on the validation set and test the performance on the leave out test set. We ensemble the prediction of the models trained on 4 splits on the same leave out test set. For the seq2seq model, since the decoding on the next primitive actually depends on the prediction of the previous step. Therefore, the prediction at a specific time step for individual model is conditioned on the average predictions of the four models from the previous step. }
%     \label{tab:my_label1}
% \end{table}



\begin{table}[]
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{ c | c  | c| c| c}
\toprule
    & \multicolumn{1}{c}{Edit Score} & \multicolumn{1}{c}{Action Error Rate} &  \multicolumn{1}{c}{FDR} & \multicolumn{1}{c}{TPR}\\
    
% \cmidrule{4-7}
%\midrule

\midrule[0.7pt]
{ Action segmentation model output }  & 62.2 (60.8 - 63.6) & 0.392 (0.371 - 0.413) &0.148 (0.135 - 0.161) &0.643 (0.622- 0.664)  \\
{Asrf (Boundary refinement)} & {58.7 (57.3 - 60.2)} & 0.436 (0.417 - 0.456) & \textbf{0.126 (0.113 - 0.139)} &  0.585 (0.566 - 0.605) \\
{Asrf (Smoothing window refinement)}  & 62.7 (61.3 - 64.1) & 0.390 (0.370, 0.410) & 0.1798 (0.166 - 0.194) &0.666 (0.646, 0.685)  \\
{Asrf (Seq2seq refinement) } & \textbf{{67.6 (66.4 - 68.8)}}& \textbf{{0.322 (0.307 - 0.339)}}  & 0.211 (0.200 - 0.221) &\textbf{{0.743} (0.732 - 0.753)}\\
\midrule[0.7pt]

{Seq2seq (on raw video feature data)} ensemble pred & {66.6 (65.4 - 67.9)} & {0.329 (0.312 - 0.345)} &0.216 (0.207 - 0.226) &0.734 (0.722 - 0.744) \\
\bottomrule
\end{tabular}
}
    \caption{Stroke video dataset: we select the model according to the best Action Error Rate (AER) on the validation set and test the performance on the leave out test set. We ensemble the prediction of the models trained on 4 splits on the same leave out test set. For the seq2seq model, since the decoding on the next primitive actually depends on the prediction of the previous step. Therefore, the prediction at a specific time step for individual model is conditioned on the average predictions of the four models from the previous step. }
    \label{tab:my_label1}
\end{table}


\begin{table}[]
\centering
% \resizebox{0.9\linewidth}{!}{
\begin{tabular}{ c | c  | c|c|c}
\toprule
    & \multicolumn{1}{c}{Edit Score} & \multicolumn{1}{c}{Action Error Rate}&  \multicolumn{1}{c}{FDR} & \multicolumn{1}{c}{TPR} \\
    
% \cmidrule{4-7}
%\midrule
\midrule[0.7pt]
{Asrf (before refinement)}  & 65.6 & 0.391&0.25 &0.75\\
{Asrf (after refinement)} & {65.7} & 0.361&0.19 & 0.70\\
{Seq2seq (on Asrf prediction)} & 63.4 &  0.36& \textbf{0.14}& 0.66\\
{Seq2seq (on raw sensor data)} & \textbf{67.8} & \textbf{0.33} & 0.17 & \textbf{0.74}\\
\bottomrule
\end{tabular}
% }
    \caption{Stroke sensor dataset}
    \label{tab:my_label1}
\end{table}

% \begin{figure}[h]

% \centering
% \includegraphics[scale=0.35]{figures/bound_acc_v_log_time.png}
% \caption{Boundary accuracy achieved by the segmentation models vs duration of the action primitives in log scale}
% \end{figure}





% \begin{table}[]
% \centering
% % \resizebox{0.9\linewidth}{!}{
% \begin{tabular}{ c | c  | c |c|c}
% \toprule
%     & \multicolumn{1}{c}{Edit Score} & \multicolumn{1}{c}{Action Error Rate} &\multicolumn{1}{c}{FDR} & \multicolumn{1}{c}{TPR} \\
    
% % \cmidrule{4-7}
% %\midrule
% \midrule[0.7pt]
% {Asrf (before refinement)}  & 69.4 & 0.47 &0.28 &\textbf{ 0.85} \\
% {Asrf (after refinement)} & 75.9 & 0.31 &\textbf{0.16} & 0.80 \\
% {Seq2seq (on Asrf prediction)} & \textbf{76.9} & \textbf{0.30} &   0.17& 0.82\\
% Seq2seq (on raw video feature data) & 69.4 & 0.54 & 0.31&0.76  \\
% \bottomrule
% \end{tabular}
% % }
%     \caption{50salads dataset}
%     \label{tab:my_label2}
% \end{table}




\begin{table}[]
\centering
% \resizebox{0.9\linewidth}{!}{
\begin{tabular}{ c | c  | c |c|c}
\toprule
    & \multicolumn{1}{c}{Edit Score} & \multicolumn{1}{c}{Action Error Rate} &\multicolumn{1}{c}{FDR} & \multicolumn{1}{c}{TPR} \\
    
% \cmidrule{4-7}
%\midrule
\midrule[0.7pt]
{Asrf (before refinement)}  & 70.8 & 0.43 &0.26 &\textbf{ 0.86} \\
{Asrf (Boundary refinement)} & 75.2 & 0.33 &\textbf{0.17} & 0.80 \\
{Asrf (Window Smoothing refinement)} & 76.4 & 0.32 & 0.18 & 0.83 \\
Asrf (Seq2seq refinement) & \textbf{76.9} & \textbf{0.30} &   0.17& 0.82\\
\midrule[0.7pt]
% {Seq2seq (on Asrf prediction)} & \textbf{76.9} & \textbf{0.30} &   0.17& 0.82\\
Seq2seq (on raw video feature data) & 69.4 & 0.54 & 0.31&0.76  \\
\bottomrule
\end{tabular}
% }
\caption{50salads dataset: following the setting in ASRF, for each fold, we use a separate small validation set divided from the training set of that fold, and test the performance on the test set of that fold. We select the model according to the best Action Error Rate (AER) on the validation set.  We then average the result of the 5 folds. }
    \label{tab:my_label2}
\end{table}




% \begin{table}[]
% \centering
% % \resizebox{0.9\linewidth}{!}{
% \begin{tabular}{ c | c  | c |c|c}
% \toprule
%     & \multicolumn{1}{c}{Edit Score} & \multicolumn{1}{c}{Action Error Rate} &\multicolumn{1}{c}{FDR} & \multicolumn{1}{c}{TPR} \\
    
% % \cmidrule{4-7}
% %\midrule
% \midrule[0.7pt]
% {Asrf (before refinement)}  & 60.9 & 1.18 & 0.35& \textbf{0.83}\\
% {Asrf (after refinement)} &  71.2  & 0.41 & 0.19& 0.77\\
% {Seq2seq (on Asrf prediction)} & \textbf{73.7} & \textbf{0.37} &\textbf{0.17}& 0.79  \\
% Seq2seq (on raw video feature data) & 64.1 & 0.55 & 0.28& 0.70\\
% \bottomrule   
% \end{tabular}
% % }
%     \caption{Breakfast dataset}
%     \label{tab:my_label3}
% \end{table}


\begin{table}[]
\centering
% \resizebox{0.9\linewidth}{!}{
\begin{tabular}{ c | c  | c |c|c}
\toprule
    & \multicolumn{1}{c}{Edit Score} & \multicolumn{1}{c}{Action Error Rate} &\multicolumn{1}{c}{FDR} & \multicolumn{1}{c}{TPR} \\
    
% \cmidrule{4-7}
%\midrule
\midrule[0.7pt]
{Asrf (before refinement)}  & 61.7 & 0.97 & 0.34& \textbf{0.82}\\
{Asrf (Boundary refinement)} &  70.9  & 0.45 & 0.19& 0.77\\
{Asrf (Window Smoothing refinement)} &  69.1  & 0.51 & 0.23& 0.79\\
Asrf (Seq2seq refinement)  & \textbf{73.7} & \textbf{0.37} &\textbf{0.17}& 0.79  \\
\midrule[0.7pt]
Seq2seq (on raw video feature data) & 64.1 & 0.55 & 0.28& 0.70\\
\bottomrule   
\end{tabular}
% }
    \caption{Breakfast dataset: following the setting in ASRF, for each fold, we use a separate small validation set divided from the training set of that fold, and test the performance on the test set of that fold. We select the model according to the best Action Error Rate (AER) on the validation set.  We then average the result of the 4 folds. }
    \label{tab:my_label3}
\end{table}




\begin{table}[]
\centering
\resizebox{1\linewidth}{!}{
% \resizebox{0.9\linewidth}{!}{
\begin{tabular}{ c | c  | c | c | c}
\toprule
    & \multicolumn{1}{c}{Edit Score} & \multicolumn{1}{c}{Action Error Rate} &\multicolumn{1}{c}{FDR} & \multicolumn{1}{c}{TPR}\\
    
% \cmidrule{4-7}
%\midrule
\midrule[0.7pt]
{Asrf (before refinement)}  & 61.44  & 0.815  & 0.357  & \textbf{0.898 }\\
{Asrf (Boundary refinement)} &  74.63   & 0.308  & 0.191  & 0.846 \\
 Asrf (Window Smoothing refinement)) & 76.54 & 0.305 & 0.174 & 0.878 \\
{Asrf (Seq2Seq refinement)} & \textbf{83.87 } &  \textbf{0.165 } &\textbf{0.092 } & 0.874  \\
 MSTCN wo cw (before refinement) & 68.48 & 0.44 & 0.269 & 0.844 \\
  MSTCN wo cw (Window Smoothing refinement)) & 72.08 & 0.335 & 0.188 & 0.807 \\
  
  MSTCN wo cw (Seq2Seq refinement) & 82.98 & 0.177 & 0.109 & 0.863 \\
\bottomrule
\end{tabular}
 }
    \caption{Jigsaws dataset}
    \label{tab:my_label3}
\end{table}









% Seq2seq on sensor data

% a. Raw features

% b. Prob. prediction of the sensor segmentation model in the seq2seq arch.

\subsection{Performance on 50salads dataset}
\label{sec:50salads_dataset}
Compare the sota model with our proposed model (a and c option).

\subsection{Performance on Breakfast dataset}
\label{sec:breakfast_dataset}
Compare the sota model with our proposed model (a and c option).

\subsection{Analysis}
\label{sec:analysis}
\subsubsection{Performance after refinement}
Show that performance for 50salads and breakfast dataset improves but for our dataset, it worsen the performance.

\subsubsection{Boundary detection performance}
Show some qualitative examples.
Think about the metric which correctly captures what we want to show.

\subsection{Short action primitives affects the boundary detection performance}
Show this for 50salads and our dataset (average length of the primitive, the boundary detection performance)

\subsection{Show some evidence that it is easy to detect boundaries in 50salads and breakfast}
Show some visual example of background.
Can we show some videos here?


\subsection{Sparse Sampling} How does sparse sampling influence the network output.

\subsection{Evidence to show that the fine-grained primitive recognition is quite local, thus does not require large receptive field}




\subsection{Baseline model}
\label{sec:baseline_model}

We select the best action segmentation model as the baseline model. ASRF is the baseline model for all the datasets. In this, we take the asrf model (adjust the hyper-parameters) and apply it to our respective data.

\subsection{Naive improvement of the baseline model}
Here we just take the outputs of the baseline asrf model which are probabilities of each class and boundary information and input them to the encoder of the LAS model. 

% \subsection{End2End finetuning the baseline model}
% \subsubsection{Using only the loss function from the decoder}
% Here the encoder will have the same architecture as ASRF (module that is used for class prediction). We can then extract the hidden vector (penultimate vector) from the two modules and pass them to the decoder. Then, train using the weighted decoder loss (where weights are decided using median freq balancing) 

% \subsubsection{Using only three loss functions (decoder loss + time-wise cel+ boundary loss)}
% Here the encoder will have the same architecture as ASRF (module that is used for class prediction). We can then extract the hidden vectors (penultimate vector) from the two modules and pass them to the decoder. Then, train using the weighted decoder loss (where weights are decided using median freq balancing). Additionally, have two more loss functions for time-wise cel and boundary cel (both weighted as per the asrf paper). 

% \subsection{Training an end2end LAS model from scratch}
% \subsubsection{Using only the loss function from the decoder}
% Using any other architecture (not restricting to ASRF model)
% \subsubsection{Using only three loss functions (decoder loss + time-wise cel+ boundary loss)}
% Using any other architecture (not restricting to ASRF model)


==> tables/act_descp_sev.tex <==
\begin{table}[t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|p{2cm}|p{3.7cm}|p{2cm}|p{3.35cm}|p{3.35cm}|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Activity}} & \multicolumn{1}{c|}{\multirow{2}{*}{Workspace}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Target \\ object(s)\end{tabular}}} & \multicolumn{2}{c|}{Instructions $^*$} \\ \cline{4-5} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Proximal \textgreater Distal} & \multicolumn{1}{c|}{Proximal \textless Distal} \\ \hline
 Washing face & Sink with a small tub in it and two folded washcloths on either side of the countertop, 30 cm from edge closest to patient & Washcloths, faucet handle & Reach to touch faucet knob. Place washcloth in paretic hand and bring to both sides of face. & Open and close faucet. Lift washcloth from basin and wring it out.  \\ \hline
 Applying deodorant & Tabletop with deodorant placed at midline, 25 cm from edge closest to patient & Deodorant & Reach to touch deodorant. Place deodorant in paretic hand and bring to opposite armpit. & Lift deodorant for 3 seconds. From the horizontal position, rotate deodorant upright and return to original position.  \\ \hline
 Hair combing & Tabletop with comb placed at midline, 25 cm from edge closest to patient & Comb & Reach to touch comb. Place comb in paretic hand and bring to both sides of head. & Lift comb for 3 seconds. \\ \hline
 Don/doffing glasses & Tabletop with glasses placed at midline, 25 cm from edge closest to patient & Glasses & Reach to touch glasses. & Lift glasses for 3 seconds. \\ \hline
Eating & Table top with a standard-size paper plate (at midline, 2 cm from edge), utensils (3 cm from edge, 5 cm from either side of plate), a baggie with a slice of bread (25 cm from edge, 23 cm left of midline), and a margarine packet (32 cm from edge, 17 cm right of midline) & Fork, knife, re-sealable sandwich baggie, slice of bread, single-serve margarine container & Reach to touch each item separately on paretic side. Place fork in paretic hand and bring fork to mouth. & Lift each object on paretic side for 3 seconds. \\ \hline
\end{tabular}}
\caption{Description of the activities performed by the severely impaired patients in the cohort (1/2). $^*$ Instructions for the severely impaired patients were given based on the UE segment with greater preserved function. “Proximal $>$ distal” indicates better strength in the proximal (i.e. deltoid, biceps, triceps) than distal (i.e. hand) UE, which was typically paralyzed in these patients. The initial UE position was generally at the edge of the table/counter closest to the patient. “Distal $>$ proximal” had the opposite distribution of strength. The initial UE position was adjacent to the target object. All testing were done on the paretic UE.}
\label{tab:sev_act_descp_1}
\end{table}

\begin{table}[t]
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{|p{2cm}|p{3.7cm}|p{2cm}|p{3.4cm}|p{3.4cm}|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Activity}} & \multicolumn{1}{c|}{\multirow{2}{*}{Workspace}} & \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Target \\ object(s)\end{tabular}}} & \multicolumn{2}{c|}{Instructions$^*$} \\ \cline{4-5} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Proximal \textgreater Distal} & \multicolumn{1}{c|}{Proximal \textless Distal} \\ \hline
Drinking & Tabletop with water bottle and paper cup 18 cm to the left and right of midline, 25 cm from edge closest to patient & Water bottle (12 oz), paper cup & Reach to touch object on paretic side. Reach across to touch object on non-paretic side. & Starting from upright position, lay object on paretic side horizontally, release, and return to upright. Perform same series of actions on the object on the non-paretic side. \\ \hline
Tooth brushing&Sink with toothpaste and toothbrush on either side of the countertop, 30 cm from edge closest to patient&Travel-sized toothpaste on left, toothbrush with built-up foam grip on right, faucet handle&Reach to touch object on paretic side. Place toothbrush in paretic hand and bring it to mouth.&Lift object on paretic side for 3 seconds. \\ \hline
Moving object on a horizontal surface&Horizontal circular array (48.5 cm diameter) of 8  targets (5 cm diameter)&Toilet paper roll (200 g) or can (200 g)&Investigator will assess if toilet paper roll can be grasped, or aluminum can if not. 
If grasp is possible, move roll/can between the center and each outer target, resting before and after each motion. 

If grasp is not possible, the toilet paper roll will be moved around the target array by the investigator and the patient will reach to touch it at each location. 
& Investigator will assess if toilet paper roll can be grasped, or aluminum can if not. 

If grasp is not possible, the toilet paper roll will be moved around the target array by the investigator and the patient will reach to touch it at each location.\\ \hline
Moving object on/off a Shelf& Shelf with two levels (33 cm and 53 cm) with 3 targets on both levels (22.5 cm, 45 cm, and 67.5 cm away from the left-most edge)&Toilet paper roll (200 g) or can (200 g)&Investigator will assess if toilet paper roll can be grasped, or aluminum can if not. 
If grasp is possible, move roll/can between the center and each outer target, resting before and after each motion. 

If grasp is not possible, the toilet paper roll will be moved around the target array by the investigator and the patient will reach to touch it at each location. 
&Investigator will assess if toilet paper roll can be grasped, or aluminum can if not. 

If grasp is not possible, the toilet paper roll will be moved around the target array by the investigator and the patient will reach to touch it at each location. \\ \hline
\end{tabular}}
\caption{Description of the activities performed by the severely impaired patients in the cohort (2/2).}
\label{tab:sev_act_descp_2}
\end{table}

==> tables/stroke_sensors_results.tex <==
\begin{table}[h]
\centering
\resizebox{1\linewidth}{!}{
% \begin{tabular}{ c|c | c  | c| c| c}
\begin{tabular}{>{\centering\arraybackslash}m{0.15\linewidth} >{\centering\arraybackslash}m{0.30\linewidth}| >{\centering\arraybackslash}m{0.20\linewidth} >{\centering\arraybackslash}m{0.22\linewidth} >{\centering\arraybackslash}m{0.22\linewidth}>{\centering\arraybackslash}m{0.22\linewidth}}
\toprule
   & Model  & {Edit Score} & {Action Error Rate} &  {FDR} &{TPR}\\
\midrule[0.7pt]
{Action}& {Baseline}  & 68.9 (67.3 - 70.5) & 0.330 (0.307 - 0.354) & 0.201 (0.186 - 0.216) & \textbf{0.790 (0.770 - 0.812)}  \\
segmentation & {+ Boundary detection } & 67.9 (66.3 - 69.5) & 0.349 (0.326 - 0.372) & 0.219 (0.205 - 0.233) &  0.784 (0.763 - 0.803) \\
model &{ + Smoothing window }  &  &  &  &  \\
\midrule[0.7pt]
\multirow{2}{*}{Seq2seq}&{Seg2seq} & 63.0 (61.3 - 64.7) & 0.337 (0.311 - 0.363)  & \textbf{0.145 (0.134 - 0.157)} & 0.707 (0.678 - 0.734)\\
&{Raw2seq} & \textbf{69.0 (67.3 - 70.6)} & \textbf{0.308 (0.287 - 0.329)} & 0.166 (0.153 - 0.179) & 0.767 (0.747 - 0.786) \\
\bottomrule
\end{tabular}
}
\caption{Comparision of seq2seq model and action segmentation model on \emph{StrokeRehab} sensor dataset: we select the model according to the best Action Error Rate (AER) on the validation set and test the performance on the leave out test set.}
    \label{tab:result_stroke_video}
\end{table}
